On the Transferability of Visually Grounded PCFGs

There has been a significant surge of interest in visually grounded grammar induction in recent times. While a variety of models have been developed for the task and have demonstrated impressive performance, they have not been evaluated on text domains that are different from the training domain, so it is unclear if the improvements brought by visual groundings are transferable. Our study aims to fill this gap and assess the degree of transferability. We start by extending VC-PCFG (short for Visually-grounded Compound PCFG~\citep{zhao-titov-2020-visually}) in such a way that it can transfer across text domains. We consider a zero-shot transfer learning setting where a model is trained on the source domain and is directly applied to target domains, without any further training. Our experimental results suggest that: the benefits from using visual groundings transfer to text in a domain similar to the training domain but fail to transfer to remote domains. Further, we conduct data and result analysis; we find that the lexicon overlap between the source domain and the target domain is the most important factor in the transferability of VC-PCFG.

==> algorithm/inside_1d_m1.tex <==
% \LinesNumberedHidden
\LinesNotNumbered
\begin{algorithm*}
% \SetAlgoLined % https://tex.stackexchange.com/a/270926 %
\caption{Inside Algorithm with Linear-sequence PCFGs}\label{alg:inside-linear}
\KwData{Input image $I$ of size $H\times W$, $\mR_1\in\mathbb{R}^{1\times N}$, $\mR_2\in\mathbb{R}^{N\times 2\times K\times K}$, $\mR_3\in\mathbb{R}^{K\times V}$, and $N = |\gN|$, $K = N + |\gP|$, and $V=|\Sigma|$.}
\KwResult{$\beta$.}
$\beta \gets \text{torch.ones(B, H, H + 1, W, W + 1, K) * -1e9}$\;

\Comment{Fill in pre-terminal rule prob.}

\For{$y\in [1,\ldots,H]$}{ 
    \For {$x\in [1,\ldots W]$} {
        $\beta[:, y, y + 1, x, x + 1] = \mR_3[:, I[y, x]][\text{None}]$
    }
}

\Comment{Linear-sequence PCFGs.}

\For{$y\in [1,\ldots,H]$}{ 
    \Comment{Inside alg. along rows (fake inside for-loop).}
    \For {$l\in [0,\ldots W]$} {
        \For {$r\in [l + 1,\ldots W]$} {
            $\beta[:, y, y + 1, l, r + 1]$ \Comment{To be filled using $\mR_2[:, 0]$.}
        }
    }
}

\For{$x\in [1,\ldots,W]$}{ 
    \Comment{Inside alg. along columns (fake inside for-loop).}
    \For {$a\in [0,\ldots H]$} {
        \For {$b\in [l + 1,\ldots H]$} {
            $\beta[:, a, b + 1, x, x + 1]$ \Comment{To be filled using $\mR_2[:, 1]$.}
        }
    }
}
\end{algorithm*} 

==> algorithm/inside_1d_m2.tex <==
% \LinesNumberedHidden
\LinesNotNumbered
\begin{algorithm*}
% \SetAlgoLined % https://tex.stackexchange.com/a/270926 %
\caption{inside\_alg\_1d($\cdot$): Inside Algorithm with Linear-sequence PCFGs}\label{alg:inside-linear}
\KwData{Input sequence $\vw$ of length $L$, $\mR_1\in\mathbb{R}^{N\times 1}$, $\mR_2\in\mathbb{R}^{N\times M\times M}$, $\mR_3\in\mathbb{R}^{T\times V}$, where $N = |\gN|$, $T = |\gP|$, $M = N + T$, and $V=|\Sigma|$.}
\KwResult{$\beta$.}
$\beta \gets \text{torch.ones}(L, L + 1, N) * -1e9$\;

% \Comment{Linear-sequence PCFGs.}

\Comment{For every span length.}
\For{$l\in [2,\ldots,L]$}{ 
    \Comment{For every span start point.}
    \For {$s\in [0,\ldots L - l]$} { 
        \Comment{For every span split point.}
        \For {$k\in [1,\ldots l - 1]$} { 
            $\beta_l = \beta[s, s + k]$
            
            $\beta_r = \beta[s + k, s + l]$
            
            $\beta[s, s + l]$ \Comment{To be filled using $\beta_1$, $\beta_2$, $\mR_2$, and $\mR_3$.}
        }
    }
}
\end{algorithm*} 

==> algorithm/inside_2d_m1.tex <==
\begin{algorithm*}
\caption{Naive Model: Inside Algorithm w/ 2D iPCFGs}\label{alg:inside-m1}
\KwData{$\beta$, $R1\in\mathbb{R}^{1\times K}$, $R4\in\mathbb{R}^{K\times K\times K}$, $R4\in\mathbb{R}^{K\times V}$, $R4\in\mathbb{R}^{K\times K\times K\times K\times K}$, and $K$ equals to $|\mathcal{N}|$.}
\KwResult{The likelihood $ll$.}

% \Comment{Fill in the chart.}

\For{$h\in [2,\ldots,H + 1]$}{ 
    \For{$w\in [2,\ldots,W + 1]$}{ 
        \For{$y\in [1,\ldots,H + 1 - h]$}{ 
            \For{$x\in [1,\ldots,W + 1 - w]$}{ 
            \Comment{All possible ways of composing a given rectangle.}

            \Comment{Case 1: fix $y$ while varying $x$.}
                \For{$s\in [1,\ldots,h]$}{ 
                    \For{$a\in [1,\ldots,w]$}{ 
                        \For{$b\in [1,\ldots,w]$}{ 
                            $b00 = \beta[:, y, y + s, x, x + a]$
                            
                            $b01 = \beta[:, y, y + s, x + a, x + w]$
                            
                            $b10 = \beta[:, y + s, y + h, x, x + b]$
                            
                            $b11 = \beta[:, y + s, y + h, x + b, x + w]$
                            
                            \Comment{Store intermediate beta's.}
                            \Comment{Can't use einsum as beta is in log domain.}
                            $// beta = \text{torch.einsum}("bi, bj, bk, bl, bsijkl", b00, b01, b10, b11, R)$
                        }
                    }
                }
            \Comment{Case 2: fix $x$ while varying $y$.}
                \For{$s\in [1,\ldots,w]$}{ 
                    \For{$l\in [1,\ldots,h]$}{ 
                        \For{$r\in [1,\ldots,h]$}{ 
                            $b00 = \beta[:, y, y + l, x, x + s]$
                            
                            $b01 = \beta[:, y, y + r, x + s, x + w]$
                            
                            $b10 = \beta[:, y + l, y + h, x, x + s]$
                            
                            $b11 = \beta[:, y + r, y + h, x + s, x + w]$
                            
                            \Comment{Store intermediate beta's.}
                            % \Comment{Can't use einsum as beta is in log domain.}
                            $// beta = \text{torch.einsum}("bi, bj, bk, bl, bsijkl", b00, b01, b10, b11, R)$
                        }
                    }
                }

            \Comment{Case 3: remove duplicate computations for $x = y$.}
                \For{$j\in [1,\ldots,h]$}{ 
                    \For{$i\in [1,\ldots,w]$}{ 
                            $b00 = \beta[:, y, y + j, x, x + i]$
                            
                            $b01 = \beta[:, y, y + j, x + i, x + w]$
                            
                            $b10 = \beta[:, y + j, y + h, x, x + i]$
                            
                            $b11 = \beta[:, y + j, y + h, x + i, x + w]$

                            \Comment{Store intermediate beta's.}
                            % \Comment{Can't use einsum as beta is in log domain.}
                            $// beta = \text{torch.einsum}("bi, bj, bk, bl, bsijkl", b00, b01, b10, b11, R)$
                    }
                }
            $\beta[:, y, y + h, x, x + w]$ \Comment{To be filled.}
            }
        }
    }
}
$ll = (\beta[:, 0, H, 0, W] + R1)\text{.logsumexp}(-1)$

\end{algorithm*}

==> algorithm/inside_2d_m2.tex <==
\begin{algorithm*}
\caption{inside\_alg\_2d($\cdot$): Inside Algorithm with iPCFGs}\label{alg:inside-m2}
\KwData{Input image $\mI\in\mathbb{R}^{H\times W}$, $\mR_1\in\mathbb{R}^{N\times 1}$, $\mR_2\in\mathbb{R}^{N\times 2\times M\times M}$, $\mR_3\in\mathbb{R}^{T\times V}$, where $N = |\gN|$, $T = |\gP|$, $M = N + T$, and $V=|\Sigma|$.}
\KwResult{The likelihood $ll$.}

$\beta \gets \text{torch.ones}(1, H, H + 1, W, W + 1, N) * -1e9$\;

% \Comment{Fill in the chart.}

\Comment{Fill in rows.}
\For{$y\in [0,\ldots,H - 1]$}{ 
    % $\beta_y = \beta[:, y, y + 1]$
    
    $\beta[:, y, y + 1] = \text{inside\_alg\_1d}(\mR_2[:, 0], \mR_3, I[y])$
}

\Comment{Fill in columns.}
\For{$x\in [0,\ldots,W - 1]$}{ 
    % $\beta_x = \beta[..., x, x + 1, :]$
    
    $\beta[..., x, x + 1, :] = \text{inside\_alg\_1d}(\mR_2[:, 1], \mR_3, \mI[:, x])$
}

\Comment{Fill in areas >= 2 x 2.}
\For{$h\in [2,\ldots,H + 1]$}{ 
    \For{$w\in [2,\ldots,W + 1]$}{ 
        \For{$y\in [1,\ldots,H + 1 - h]$}{ 
            \For{$x\in [1,\ldots,W + 1 - w]$}{ 
            \Comment{All possible ways of composing a given rectangle.}

            \Comment{Case 1: horizontal composition.}
                \For{$s\in [1,\ldots,w]$}{ 
                    $\beta_l = \beta[:, y, y + h, x, x + s]$

                    $\beta_r = \beta[:, y, y + h, x + s, x + w]$

                    \Comment{Store intermediate beta's.}
                    \Comment{Can't use einsum as beta is in log domain.}
                    $// beta = \text{torch.einsum}("bi, bj, bsij", \beta_l, \beta_r, \mR_2[:, 0])$
                }
            \Comment{Case 2: vertical composition.}
                \For{$s\in [1,\ldots,h]$}{ 
                    $\beta_t = \beta[:, y, y + s, x, x + w]$

                    $\beta_b = \beta[:, y + s, y + h, x, x + w]$

                    \Comment{Store intermediate beta's.}
                    % \Comment{Can't use einsum as beta is in log domain.}
                    $// beta = \text{torch.einsum}("bi, bj, bsij", \beta_t, \beta_b, \mR_2[:, 1])$
                }
            \Comment{Stack all the intermediate beta's}
            \Comment{and apply {logsumexp} along the new axis.}
            $\beta[:, y, y + h, x, x + w]$ \Comment{To be filled.}
            }
        }
    }
}
$ll = (\beta[:, 0, H, 0, W] + \mR_1)\text{.logsumexp}(-1)$

\end{algorithm*}

==> figure/data_analysis_rule_to_wsj.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=.95\linewidth]{figure/data_analysis/rule_cover_rate_to_wsj.pdf}
\caption{\label{fig:rule-type}
Overlap rates for rules (broken down per rule type) between the WSJ test set and the MSCOCO (WSJ-L10) training set (see results on Brown and Enweb in Figure~\ref{fig:data-analysis-lrw-rule-ood}).
}
\end{figure}

==> figure/data_analysis_success_to_failure_wsj.tex <==
\begin{figure*}[t]
\centering

\begin{minipage}[c]{0.65\textwidth}
\begin{subfigure}{.5\linewidth}
    \includegraphics[width=1.\linewidth]{figure/success_to_failure/ratio_of_success_to_failure_bucket_wsj.pdf}
    % \caption{.}
    \label{fig:s2f-bucket-wsj}
\end{subfigure}
\hfill
\begin{subfigure}{.5\linewidth}
    \includegraphics[width=1.\linewidth]{figure/success_to_failure/ratio_of_success_to_failure_wsj.pdf}
    % \caption{.}
    \label{fig:s2f-wsj}
\end{subfigure}
\end{minipage}\hfill
\begin{minipage}[c]{0.275\textwidth}
\vspace{-2.25em}
\caption{\label{fig:data-analysis-s2f-wsj}
The ratio of success to failure for each sentence length bucket (left) and for individual sentence lengths (right).
The $Y$ axis at zero indicates that \tvcpcfg makes zero mistakes.
}
\end{minipage}

\end{figure*}

==> figure/label_by_length_distributions.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}{.47\linewidth}
    \includegraphics[width=1.\linewidth]{figure/lspan_label/lspan_label_dist_mscoco_train.pdf}
    \caption{MSCOCO Training Set.}
    \label{fig:ms-train}
\end{subfigure}
\hfill
\begin{subfigure}{.47\linewidth}
    \includegraphics[width=1.\linewidth]{figure/lspan_label/lspan_label_dist_wsj_train_l10.pdf}
    \caption{WSJ L10 Training Set.}
    \label{fig:wsjl10-train}
\end{subfigure}%
\\
\vspace{2mm}
\begin{subfigure}{.47\linewidth}
    \includegraphics[width=1.\linewidth]{figure/lspan_label/lspan_label_dist_mscoco_test.pdf}
    \caption{MSCOCO Test Set.}
    \label{fig:ms-test}
\end{subfigure}%
\hfill
% \begin{subfigure}{.47\linewidth}
%     \includegraphics[width=1.\linewidth]{figure/lspan_label_dist_eng_test.pdf}
%     \caption{WSJ Test Set.}
%     \label{fig:wsj-test}
% \end{subfigure}
\begin{subfigure}{.47\linewidth}
    \includegraphics[width=1.\linewidth]{figure/lspan_label/lspan_label_dist_flickr_test.pdf}
    \caption{Flickr Test Set.}
    \label{fig:flickr-test}
\end{subfigure}
\\
\vspace{2mm}
\begin{subfigure}{.47\linewidth}
    \includegraphics[width=1.\linewidth]{figure/lspan_label/lspan_label_dist_brown_train-l10.pdf}
    \caption{Brown L10 Training Set.}
    \label{fig:brownl10-train}
\end{subfigure}
\hfill
\begin{subfigure}{.47\linewidth}
    \includegraphics[width=1.\linewidth]{figure/lspan_label/lspan_label_dist_brown_test.pdf}
    \caption{Brown Test Set.}
    \label{fig:brown-test}
\end{subfigure}%
\\
\vspace{2mm}
\begin{subfigure}{.47\linewidth}
    \includegraphics[width=1.\linewidth]{figure/lspan_label/lspan_label_dist_enweb_train-l10.pdf}
    \caption{Enweb L10 Training Set.}
    \label{fig:enwebl10-train}
\end{subfigure}%
\hfill
\begin{subfigure}{.47\linewidth}
    \includegraphics[width=1.\linewidth]{figure/lspan_label/lspan_label_dist_enweb_test.pdf}
    \caption{Enweb Test Set.}
    \label{fig:enweb-test}
\end{subfigure}
\caption{\label{fig:efficiency-length}
Phrasal label distribution broken down per constituent length.
}
\end{figure*}

==> figure/mscoco_to_others_l10.tex <==
\begin{figure*}[t]
\centering

\includegraphics[width=1\linewidth]{figure/mscoco_to_others/mscoco_to_others_f1_l10.pdf}

\caption{\label{fig:mscoco-to-others-f1}
S-F1 numbers of .
}
\end{figure*}

==> figure/mscoco_to_others_tc.tex <==
\begin{figure*}[t]
\centering

\includegraphics[width=1\linewidth]{figure/mscoco_to_others/mscoco_to_others_f1_tc.pdf}

\caption{\label{fig:mscoco-to-others-f1}
S-F1 numbers of .
}
\end{figure*}

==> figure/recall_by_len_ood.tex <==
% \begin{figure}[t]
% \centering

% \includegraphics[width=1\linewidth]{figure/recall_by_len_wsjl10.pdf}

% \caption{\label{fig:rule-type}
% Recall broken down per constituent length.
% }
% \end{figure}

\begin{figure*}[t]
\centering
\begin{subfigure}{.49\linewidth}
    \includegraphics[width=1.\linewidth]{figure/lspan_label/lspan_label_dist_wsj_test.pdf}
    \caption{WSJ Test Set.}
    \label{fig:label-dist-test-wsj}
\end{subfigure}
\hfill
\begin{subfigure}{.49\linewidth}
    \includegraphics[width=1.\linewidth]{figure/lspan_label/recall_by_len_test_wsj.pdf}
    \caption{WSJ Test Set.}
    \label{fig:recall-per-length-test-wsj}
\end{subfigure}
% \hfill
\\
\vspace{2mm}
\begin{subfigure}{.49\linewidth}
    \includegraphics[width=1.\linewidth]{figure/lspan_label/lspan_label_dist_brown_test.pdf}
    \caption{Brown Test Set.}
    \label{fig:label-dist-test-brown}
\end{subfigure}
\hfill
\begin{subfigure}{.49\linewidth}
    \includegraphics[width=1.\linewidth]{figure/lspan_label/recall_by_len_test_brown.pdf}
    \caption{Brown Test Set.}
    \label{fig:recall-per-length-test-brown}
\end{subfigure}
% \hfill
\\
\vspace{2mm}
\begin{subfigure}{.49\linewidth}
    \includegraphics[width=1.\linewidth]{figure/lspan_label/lspan_label_dist_enweb_test.pdf}
    \caption{Enweb Test Set.}
    \label{fig:label-dist-test-enweb}
\end{subfigure}
\hfill
\begin{subfigure}{.49\linewidth}
    \includegraphics[width=1.\linewidth]{figure/lspan_label/recall_by_len_test_enweb.pdf}
    \caption{Enweb Test Set.}
    \label{fig:recall-per-length-test-enweb}
\end{subfigure}
% \hfill
\caption{\label{fig:recall-by-len-ood}
Phrasal-label distributions (left column) and recall (right column) broken down per constituent length.
}
\end{figure*}

==> section/robustness.tex <==
\subsection{Model Variance}

In both the results reported by~\citet{zhao-titov-2020-visually} and our transfer learning results, we observe high variances in the performance of \vcpcfg. 
% Though neural PCFG models exhibit large performance variances on their own~\citep{kim-etal-2019-compound,zhao-titov-2021-empirical},
% Though non-grounded grammar models such as neural PCFGs, PRPN, ON-LSTM exhibit some performance variances on MSCOCO captions on their own~\citep{shen2018neural,shen2018ordered,kim-etal-2019-compound,zhao-titov-2021-empirical},
Though non-grounded grammar models such as neural \pcfg exhibit some variances on their own~\citep{kim-etal-2019-compound,zhao-titov-2021-empirical},
this observation raises doubts about how significantly visual groundings improve grammar induction.
To clear the doubts, we further investigate the variances of \vcpcfg. We identify two sources of randomness in training: model initialization and data order (i.e., in which order the training data is present). We conduct statistical significance tests and find that \vcpcfg improves over \cpcfg by 1.9\% sentence-level F1 at a significance level of 0.1.

% \subsubsection{Model Variance}

\input{table/randomness.tex}

We observe that all the grammar models based on \cpcfg exhibit high variance\footnote{Besides \pcfg-based models, PRPN~\citep{shen2018neural} and ON-LSTM~\citep{shen2018ordered} show high variance on MSCOCO captions (see Table~\ref{tab:transfer_mscoco}).} across different runs on all datasets, which makes the results hard to explain. For example, replacing learnable word embeddings with pre-trained Glove makes \cpcfg worse than the right-branching baseline but improves \vcpcfg by 6.9\% S-F1 (see Table~\ref{tab:transfer_mscoco}).
On Flickr30k, surprisingly, \cpcfg outperforms \vcpcfg, which indicates that visual groundings deteriorate model performance on this dataset, but results on MSCOCO suggest the opposite~\citep{zhao-titov-2020-visually}.
Considering the large variances, it is unclear
if the improvements over the non-grounded parser brought by visual groundings are statistically significant.
% if visual groundings really help with grammar induction significantly. %, or if it is just because of lucky random seeds.

To investigate the high-variance issue, we first identify two sources of randomness: (1) model initialization, i.e., random seeds that are used to initialize models (RM); and (2) data order, i.e., in which order training samples are present to models (RD). 
We design controlled experiments to study the role of the two types of randomness:
\begin{itemize}
    \item \textbf{RM+RD:} we train \cpcfg with both different initializations and different random data orders.
    \item \textbf{RM:} we train \cpcfg with different initializations but keep the same data order.
    \item \textbf{V-RM:} we train \vcpcfg with different initializations but keep the same data order
\end{itemize}
% (1) we train \cpcfg with both different initializations and different random data orders (RM+RD); (2) we train \cpcfg with different initializations but keep the same data order (RM); and (3) we train \vcpcfg with different initializations but keep the same data order (V-RM). 
To obtain relatively sufficient statistics, we run each experiment 12 times with different random seeds on MSCOCO. For the same random seed, we make sure that all the parsing models have the same initialization.\footnote{\vcpcfg has an additional image-caption matching module compared with \cpcfg.}

Ideally, RM+RD and RM should have similar performance because they are trained on the same set of training data. However, our results show that RM performs better than RM+RD in terms of mean F1 scores (see Table~\ref{tab:randomness}), i.e., \cpcfg is sensitive to the order of training data, which is not expected.
Comparing V-RM and RM, we can see that visual groundings improve \cpcfg trained only on text (+2.1\% S-F1), but given the high model variance (i.e., around 12\% in terms of the standard deviation), it is unclear if these improvements are statistically significant.
% it is not immediately clear that visual groundings contribute to the improvements significantly. 

To assess if the difference between RM and RM+RD and the difference between RM and V-RM are significant, we conduct Paired T-Test (see the second section of Table~\ref{tab:randomness}). 
%Given $t_{0.05, 11} = 2.201$,\footnote{$t_{0.05, 11} = 2.201$ means that the $t$ value with $\alpha=0.05$ (i.e., $p$-value) and 11 degrees of freedom is 2.201. A $t$-value larger than $t_{0.05, 11}$ means that we reject the null hypothesis that there is no difference between the means of two groups.} 
At a significance level of 0.1, i.e., $\alpha=0.1$, we, unfortunately, fail to reject the null hypothesis that there is no difference between the means of RM and RM+RD (\emph{p} > $\alpha$), but we reject the null hypothesis for RM and V-RM (\emph{p} < $\alpha$). 
% for every column / pair of groups. 
In other words, 
\begin{itemize}
	\item The training data order seems to have a big influence on model performance but in fact, does not make a \emph{significant} difference.
	\item Visual groundings 
 % seem helpful but do not 
 make a \emph{significant} influence on parsing performance. On average, they improve \cpcfg by 1.9\% S-F1.
\end{itemize}
% (DELETED) However, if we slightly relax the level of significance to 0.1, visual groundings indeed \emph{significantly} improve over a non-grounded C-PCFG for NPs and VPs. If we consider the One-Tailed Test, the improvements on NPs and VPs are \emph{significant} at the significance level of 0.05, but why the conclusion is different from Two-Tailed T-Test.\footnote{For One-Tailed Paired T-Test, the null hypothesis $H_0=\text{there is no difference in means of RI and V-RI}$, and the alternative hypothesis $H_1=\text{V-RI has a larger mean than RI}$.}

To give a more intuitive explanation of significance tests, we compute performance differences for paired experiments and report their mean and standard deviation (see the last section of Table~\ref{tab:randomness}). Take V-RM and RM, the average difference (+1.9\% F1), which indicates the average improvement of V-RM over RM, is quite small because, for some random seeds, V-RM performs better but, for others, it underperforms RM.
Though they both show high variances (12.1\% vs 13.4\% std), the variance of paired differences is much smaller (\emph{cf.} 3.6\% std), which means that the improvement of V-RM over RM is relatively reliable.

==> table/randomness.tex <==
\begin{table*}[t!]\small
	\centering
	{\setlength{\tabcolsep}{.65em}
		\makebox[\linewidth]{\resizebox{\linewidth}{!}{%
				\begin{tabular}{rllllllll}
					\toprule
					\multicolumn{1}{r}{\textbf{Model}} &
					\multicolumn{1}{l}{\textbf{NP}} & 
					\multicolumn{1}{l}{\textbf{VP}} & 
					\multicolumn{1}{l}{\textbf{PP}} & 
					\multicolumn{1}{l}{\textbf{SBAR}} & 
					\multicolumn{1}{l}{\textbf{ADJP}} & 
					\multicolumn{1}{l}{\textbf{ADVP}} & 
					\multicolumn{1}{l}{\textbf{C-F1}} & 
					\multicolumn{1}{l}{\textbf{S-F1}} \\
					\midrule
					RM+RD & 53.0$_{\pm 25.2}$ & 64.0$_{\pm 21.9}$ & 67.6$_{\pm 8.2}$ & 77.4$_{\pm 11.6}$ & 65.0$_{\pm 9.5}$ & 83.5$_{\pm 4.0}$ & 52.4$_{\pm 12.4}$ & 52.9$_{\pm 12.6}$ \\
					RM & 58.2$_{\pm 27.8}$ & 62.7$_{\pm 21.2}$ & 67.0$_{\pm 6.2}$ & 76.1$_{\pm 12.3}$ & 52.7$_{\pm 18.7}$ & 81.3$_{\pm 8.6}$ & 54.3$_{\pm 13.3}$ & 54.7$_{\pm 13.4}$ \\
					V-RM &  59.5$_{\pm 24.4}$ & 66.3$_{\pm 22.0}$ & 70.1$_{\pm 7.1}$& 77.1$_{\pm 13.0}$& 61.4$_{\pm 15.0}$& \text{83.9}$_{\pm 6.6}$& 56.2$_{\pm 12.0}$& 56.6$_{\pm 12.1}$\\
					\midrule
					\multicolumn{9}{c}{\emph{p}-values from the Two-Tailed Paired T-Test} \\
     % {\color{(white!75}{divided by 2 for One-Tailed T-Test)}}}\\
					\cmidrule{2-8}
					RM+RD \emph{vs} RM &	0.588&	0.846&	0.710&	0.720&	0.067&	0.280 & 0.641	& \cellcolor{myorange!25}0.647 \\
					V-RM \emph{vs} RM &	0.464&	0.306&	0.064&	0.625&	0.060&	0.096 & 0.083&	\cellcolor{blue!25}0.095\\
					\midrule
					\multicolumn{9}{c}{\emph{mean} and \emph{std} of performance differences between paired experiments} \\
     % {\color{(white!75}{divided by 2 for One-Tailed T-Test)}}}\\
					\cmidrule{2-8}
					RM+RD $-$ RM & -5.1$_{\pm 31.9}$ & 1.3$_{\pm 22.7}$ & 0.6$_{\pm 5.4}$ & 1.3$_{\pm 12.2}$ & 12.4$_{\pm 21.1}$ & 2.3$_{\pm 7.0}$ & -1.9$_{\pm 13.7}$ & \cellcolor{myorange!25}-1.9$_{\pm 13.9}$ \\
					V-RM $-$ RM & \phantom{-}1.4$_{\pm 6.2}$ & 3.7$_{\pm 11.8}$ & 3.1$_{\pm 5.2}$ & 1.0$_{\pm 7.0}$ & \phantom{0}8.7$_{\pm 14.4}$ & 2.6$_{\pm 5.0}$ & \phantom{-}2.0$_{\pm 3.6}$ & \cellcolor{blue!25}\phantom{-}1.9$_{\pm 3.6}$ \\
%					\multicolumn{9}{c}{\emph{t}-values from the Paired T-Test ($t_{0.05, 11} = 2.201$)}\\
%					\cmidrule{3-7}
%					RI+RD \emph{vs} RI & 0.480 &	0.470 &	0.558&	0.199&	0.381&	0.367&	2.031&	1.137 \\
%					RI \emph{vs} V-RI & 0.759 & 1.074 &	2.057 &	0.503 &	2.098 &	1.817 & 1.903 &	1.828\\
					\bottomrule
	\end{tabular}}}}
	\caption{\label{tab:randomness}
		Controlled experiments. RM and RD are short for `random model initialization' and `random data order', respectively. They are both applied to \cpcfg (RM+RD). V-RM represents a \vcpcfg with the same settings as RM but is additionally trained with the image-caption alignment loss. 
		%A $t$-value larger than $t_{0.05, 11}= 2.201$ means that we reject the null hypothesis that there is no difference between the means of two groups.
	}
\end{table*}
